Automatic Curriculum Learning through Value Disagreement

Continually solving new, unsolved tasks is the key to learning diverse behaviors. Through reinforcement learning (RL), we have made massive strides towards solving tasks that have a single goal. However, in the multi-task domain, where an agent needs to reach multiple goals, the choice of training goals can largely affect sample efficiency. When biological agents learn, there is often an organized and meaningful order to which learning happens. Inspired by this, we propose setting up an automatic curriculum for goals that the agent needs to solve. Our key insight is that if we can sample goals at the frontier of the set of goals that an agent is able to reach, it will provide a significantly stronger learning signal compared to randomly sampled goals. To operationalize this idea, we introduce a goal proposal module that prioritizes goals that maximize the epistemic uncertainty of the Q-function of the policy. This simple technique samples goals that are neither too hard nor too easy for the agent to solve, hence enabling continual improvement. We evaluate our method across 13 multi-goal robotic tasks and 5 navigation tasks, and demonstrate performance gains over current state-of-the-art methods.

==> broader_impacts.tex <==
\section{Broader Impact}

While recent advancements in Artificial Intelligence (AI) provide a lot of potential opportunities to create products such as in elderly care, medical consultant and surgery assistant, autonomous devices that keep the supply chain sustainable under extreme working conditions or during pandemic, etc. It also provides tools that utilize the availability of large amount of data today, with the end-goal of improving our quality of life. There are however multiple possible negative consequences that we must be aware of: (i) training neural networks is typically associated with large energy consumption that is harmful to the environment, (ii) the significant computation resource requirement prevents many researchers from accessing state-of-the-art research, and (iii) in the field of RL in particular, algorithms typically require a long duration of interaction with the environments, which could further introduce a prohibitive monetary cost when deployed on physical robotic environments. In this paper, we focus on improving sample efficiency when training a universal agent that can perform a range of tasks. Furthermore, VDS is accessible to a broad range of researchers (even those without access to GPUs) and leaves a much smaller carbon footprint than competing methods. In fact, all of our experiments using VDS are run on a single CPU.

It is fair to say that even with the result of this paper, Deep RL agents are far from being applicable to complex problems in real life and being widely accessible to the public. Regardless, we believe this paper provides progress and contributes to the goal of making reliable robotic applications. Along this process we are aware that evaluating robot safety is a crucial part of the consideration. Therefore rather than exclusively focusing on developing state-of-the-art algorithms, we draw attention to complementary research on safety~\cite{AmodeiOSCSM16, irving2019safety}. 

==> teacher-student.tex <==

\subsection{Teacher's POMDP Formulation}
\label{sec:teacher-student}
\lpnote{Remove POMDP mention to avoid confusing reader.}
\lpnote{Two MDPs. One for Student. One for Teacher. Superscript with S or T respectively.}
We formulate the Teacher's POMDP similar to ~\cite{} but with a different reward function, which is designed to be equipped with a convenient update rule \ref{eq:teacher_update} which falls back into the standard Bellman updates, relying completely on the experience data collected by the Student and does not require extra interaction with the environment.\lpnote{Break prev. sentence down.}

\begin{itemize}
    \item \textbf{State Space}
    Denote the state space for the Teacher as $\Pi$, defined as the parameter space of the Student's policy $\pi$. The Student is treated as an unobservable black box RL algorithm and thus dropped from the POMDP representation. 
    
    TODO: the assumption that the student is "unobservable" is actually incorrect because the Teacher sees the full replay buffer? Also in POMDP does Q takes in the state, in this case $\bar{Q}(\pi, g)$, or just $\bar{Q}(g)$?
    \item \textbf{Action space}
    The Teacher's action is to propose a goal $g$ in the goal space $\mathcal{G}$, and the Student will play rollouts conditioned on $g$ in the next training epoch. We denote the action space as $\mathcal{G}$. \lpnote{Use proper }
    \item \textbf{Horizon}
    The horizon for the POMDP is $1$, because we only care about the performance of the latest Student's policy. The Teacher's transitional probability is dropped form the MDP representation since the episode restarts after every timestep of the Teacher. \lpnote{make it crisper}
    
    \item \textbf{Reward}
    The reward for the Teacher is the negative episodic reward of the Student. Formally, let $\mathcal{M}_S = (\mathcal{S}\times\mathcal{G}, \mathcal{A}, \mathcal{T}, R, T, \rho_s\times\rho_g)$ be the MDP for the Student as in standard Multigoal RL, where $\mathcal{T}$ is the transition probability, $R$ is the reward function, $T$ is the horizon, and $\rho_s$ and $\rho_g$ are the initial goal and state distributions respectively. 
    Let $\pi$ be the Student's policy. Define the Teacher's reward given $\pi\in \Pi, g\in \mathcal{G}$ as $\bar{R}(\pi, g) = - \E_{s_0\sim\rho_0, a_t\sim\pi(\cdot \mid s_t, g), s_{t+1}\sim\mathcal{T}(\cdot\mid s_t, a_t)}\left[\sum_{t=0}^{T-1} \gamma^t R(s_t, g, a_t)\right]$. 
    
    % Comments: the definition of $\bar{R}$ also relies on $\pi$, which is a bit problematic. We can formulate the Teacher as POMDP with $\pi$ in state space but not observable. But then the transitional probability is not well-defined? 


\end{itemize}
Distinct from previous Teacher-Student POMDP formulation, we take a Beyesian view of the Teacher's POMDP. Let $\mathcal{S}, \mathcal{A}, \mathcal{G}$ be fixed. Thus far we can write the Teacher's POMDP as
\begin{equation}
    \label{eq:teacher_mdp}
    \mathcal{M}_T = (\Pi, \mathcal{G}, \bar{\mathcal{T}}, \bar{R}) \in (\Omega, \mathcal{F}, \mathbb{P})
\end{equation}
where $(\Omega, \mathcal{F}, \mathbb{P})$ is a probability space. 

\subsubsection{Q-function update for the Teacher}

Let $Q^*$ be the optimal Q-function for the Teacher's POMDP $\mathcal{M}_T = (\Pi, \mathcal{G}, \bar{\mathcal{T}}, \bar{R})$, then it satisfies the Bellman's equation in the special case of horizon length $1$: 
\begin{equation}
    \label{eq:teacher_bellman}
    \bar{Q}^*(\pi, g) = \bar{R}(\pi, g)
\end{equation}

Note that $\mathcal{M}_T$ is in one-to-one correspondence with $\bar{Q}^*$. Inspired by ~\cite{}, we use the ensemble $\{\bar{Q}_k\}_{k=1}^K$ to approximate the prior of $\bar{Q}^*$ which is typically intractable. At iteration $i+1$, the update rule for $\bar{Q}_{k, i+1}$ after seeing transition $\tau = (g, \hat{R})$ is 
\begin{equation}
    \label{eq:teacher_update}
    \bar{Q}_{k, i+1} \leftarrow \argmin_{\bar{Q}_{k, i+1}} \E_{\bar{\mathcal{T}}\sim\Tilde{p}\left(\bar{\mathcal{T}}\mid\bar{Q}_{k, i}, \tau\right)} \left[\bar{Q}_{k, i+1}(\pi, g) - \hat{R}\right]^2
\end{equation}
which maximizes the lower-bound of the posterior distribution $\Tilde{p}(Q_{k, i+1}, \bar{\mathcal{T}}\mid\tau)$. The derivation is similar to ~\cite{}. The optimization objective in \ref{eq:teacher_update} can be simplified as $\left[\bar{Q}_{k, i+1}(\pi, g) - \hat{R}\right]^2$.

Let $Q^\pi$ be the Q-function of the Student. Since $\hat{R}$ is an empirical sample of $\bar{R}(\pi, g)$, the empirical mean of $\hat{R}$ converges to $\bar{R}(\pi, g)$. Thus $\bar{R}(\pi, g) = \E_{s \sim \rho_s(\cdot)}\left[-Q^\pi (s, \pi(s), g)\right]$ is an unbiased estimator of the minimizer of \ref{eq:teacher_update}. [Is this right??] The update rule for $Q_k$ becomes
\begin{equation}
    \bar{Q}_{k, i+1} \leftarrow \E_{s \sim \rho_s(\cdot)}\left[-Q^\pi (s, \pi(s), g)\right]
\end{equation}


\subsubsection{Exploration strategy for the Teacher}
Let $\Tilde{\mu}(\pi, g)$ and $\Tilde{\delta}(\pi, g)$ be the empirical mean and standard deviation of $\{\bar{Q}_k(\pi, g)\}_{k=1}^K$. Similar to ~\cite{}, we extend UCB algorithms to the MDP of the Teacher. Namely, the Teacher takes an action $g$ according to the expected reward with a exploration bonus,
\begin{equation}
    \label{eq:ucb}
    g \in \argmax_g{\Tilde{\mu}(\pi, g) + \lambda \Tilde{\delta}(\pi, g)}
\end{equation}
with hyperparameter $\lambda \in \R_+$. 

Note that the first term in \ref{eq:ucb} is the negative episodic reward for the Student, and thus the Teacher tends to propose goals which the Students are not yet able to achieve.

The second term is a proxy for the uncertainty of the Teacher. Empirically, a goal with high uncertainty tends to lie on the boundary of the Student's solvable region as suggested by \ref{fig:heatmap}, thereafter automatically setting up the curriculum. 

Our formulation is distinct from previous works on Teacher-Student style curriculum learning, as we don't explicitly measure the learning progress (LP) of the Student, which either targets only at discrete tasks ~\cite{} or requires nearest-neighbor computation ~\cite{} that introduces extra computation burden to the Teacher \yznote{although our method requires training extra Q networks too}. Rather, the Teacher receives reward as a function only of the Student's most recent performance. 

The learning progress of the Student is implicitly captured in the epistemic uncertainty of the Teacher's value function. When the Student makes significant progress or suffers from catastrophic forgetting in some subspace of $\mathcal{G}$, the epistemic uncertainty increases due to the inconsistency in the historical data $\mathcal{H}_T = \{(g_t, \hat{R}_t)\}_t$ that the Teacher has observed, where $t$ is the Teacher's epoch index. 

\yznote{Do we want to A. provide the intuition of the Students's knowledge boundary first, and then introduce value function variance as a proxy, and cast into the language of UCB, or B. use UCB. to motivate value function variance, and then say that it maps in to the intuition? Current approach is B. }

\subsection{Goal Proposal Module}
Denote the teacher's stochastic policy as $\mathcal{C}: \mathcal{G} \rightarrow \R$, a probability distribution over Teacher's action space $\mathcal{G}$. In standard goal-conditioned RL, $\mathcal{C}(\cdot)$ reduces to the uniform distribution. However, sampling goals uniformly is often uninformative for the learning process~\cite{andrychowicz2017hindsight} since during the early stages of learning, the sampled goals are too hard, while during the later stages of learning the sampled goals are too easy. Instead of using a uniform distribution over the goals, curriculum learning based approaches sample goals in increasing order of difficulty. 

% Ideally, the samples from the $\mathcal{C}$ should lie at the frontier of learning, i.e. goals that are neither too easy nor too hard. To account for this, we condition the goal proposal module on the current policy and represent it as:

% \begin{equation}
%     \label{eq:GPM}
%     g \sim \mathcal{C}_k(\mathbb{G}; \pi^k)
% \end{equation}

We note that this formalism of the Goal Proposal Module is not limited to Student-Teacher style curriculum learning. For example, for goal generation curriculum learning ~\cite{florensa2017reverse}, $\mathcal{C}(g) = \mathbb{P}(G(z) = g)$ where $G$ is a generator network that generates goal of appropriate difficulty, and $z$ follows the prior distribution. For goal swapping in hindsight, ~\cite{andrychowicz2017hindsight}, $\mathcal{C}(g) \propto \mathbb{I}_{\mathbb{S}_\mathrm{future}}(g)$ where $\mathbb{S}_\mathrm{future}$ is the set of achieved goals in future timesteps of the current episode and $\mathbb{I}$ is the indicator function. 

\subsection{Value disagreement}
\label{sec:method_value_disagreement}

We instantiate the results from \ref{sec:teacher-student} and cast into the framework of Goal Proposal Module as the Teacher's policy. To update $\bar{Q}_{k}$ according to $\ref{eq:teacher_update}$, $Q^\pi$ can be optimized with the standard Bellman update rule~\cite{sutton1998introduction}, 
\begin{equation}
    \label{eq:bellman}
    Q^\pi_\phi(s, g, a) \leftarrow r(s, g, a) + \gamma Q_\phi^\pi(s^\prime, g, \pi(s))
\end{equation}
which reuses the transitions collected by the Student. It does not introduce extra sample complexity and maintains the flexibility to choose any RL algorithm for the Student.

\yznote{ in our implementation we don't use $\E_{s\sim\rho_s}$. We just approximate this expectation with $s = s_0$, the actual initial state of the new episode. Not sure if we should explicitly mention this. (not too related but similar argument could be made to justify curiosity-driven approach or cast as a meta-learning problem.)}

Then we perform optimization with a softened objective for \ref{eq:ucb}. Formally, 
\begin{equation}
    \label{eq:goal_dist}
    \mathcal{C}(\pi, g) = \frac{1}{Z} \exp\{(\Tilde{\mu}(\pi, g) + \lambda\Tilde{\delta}(\pi, g))/T\}
\end{equation}
where $Z = \int_\mathcal{G} \exp\{(\Tilde{\mu}(g) + \lambda\Tilde{\delta}(g))/T\}\;\mathrm{d} g$ is the normalization constant and $T\in\R_+$ is the temperature. 

\yznote{in our implementation we don't use exp. we use square function instead (so that std becomes variance). }

To approximate $\mathcal{C}$ in the limit of $\lambda \rightarrow \infty$, we compute an empirical distribution of proposed goals $\hat{\mathcal{C}}(g) \propto \Tilde{\delta}(g)$, with $g\in \mathbb{G} = \{g^{(1)}, \cdots, g^{(l)}\} \subset \mathcal{G}$. 

\yznote{ technically $\mathcal{C}$, the policy of the Teacher, can't take in $\pi$ because it is not observable. Can say that the observation space for the Teacher is $\mathcal{H}_t$ which makes everything more accurate but not sure if it is necessary. }

In all our experiments, we use $\lambda = \infty$. We train the ensemble $\{\bar{Q}_k\}_{k=1}^K$ with different parameter initialization and independently sampled mini-batches. 

% We use the epistemic uncertainty of the Value function as the goal sampling distribution. The Value function of the policy $V^{\pi}_\phi(s, g)$ with learnable parameters $\phi$ approximates the expected cumulative return $\E_{s_0=s, \tau \sim \pi(.)}\left[\sum_{t=0}^{T-1} \gamma^t r(s_t,g)\right]$. This value function can be optimized using the Bellman update rule~\cite{sutton1998introduction}:

% \begin{equation}
%     \label{eq:bellman}
%     V^\pi_\phi(s, g) \leftarrow r(s_t, g) + \gamma V_\phi^\pi(s_{t+1}, g)
% \end{equation}

% Intuitively, this function tracks the performance of the policy $\pi$ across starting states $s \sim \mathcal{S}$ and desired goals $g \sim \mathbb{G}$.

% To estimate the epistemic uncertainty we measure the disagreement across an ensemble of parametric value functions following \cite{lakshminarayanan2017simple}. Hence instead of a single $V$, we maintain $M$ value functions $V_{1:M}$ with independently trained parameters $\phi_{1:M}$. The disagreement between value functions for a goal $g$ is computed as:

% \begin{equation}
%     \label{eq:disagreement}
%     \text{disagreement}(g;V_{1:m}) = \rho_s(\text{variance}(V_{1:m}(g)))
% \end{equation}

% where we use $\rho_s \equiv I$ the identity function for simplicity across our experiments. Effectively, given the value ensemble, the epistemic uncertainty of the solvability of a goal is computed as the variance in the prediction of individual value networks.

% The discussion on different functions mapping from value ensemble predictions to the disagreement will be deferred to  \Secref{sec:disagreement}. 


Our method is summarized in \Algref{alg:vds}. For our experiments, we use DDPG~\cite{lillicrap2015continuous} as our base RL algorithm to train the policy. In each iteration, we first sample a set of goals $g_{1:l}$ uniformly from the goal set $\mathbb{G}$. Then, we compute the value disagreement and determine the goal distribution $\mathcal{C}_k(g_{1:l})$. Goals sampled according to $\mathcal{C}_k(g_{1:l})$ are used to generate rollouts which consist of transitional data used to train both the value ensemble and the policy. 

Note that although we use an off-policy algorithm as our base optimizer, the goal sampler is independent to the choice of the base RL optimizer. The value ensemble and the policy receive the same data, but they are trained separately to maintain the independence and flexibility of the goal proposal module. 

\begin{algorithm}[tb]
   \caption{Curriculum Learning with Bayesian Teacher}
   \label{alg:vds}
\begin{algorithmic}
   \State {\bfseries Input:} RL algorithm $A$, goal set $\mathbb{G}$, replay buffer $R$. 
   \State {\bfseries Initialize:} Learnable parameters $\theta$ for $\pi_\theta$ and $\phi_{1:m}$ for $V_{1:m}$
  \For {$k$=1,2,..$N_\text{iter}$} \Comment {Teacher epoch}
  \State sample $l$ goals $g_{1:l} \sim \sG$
  \State Compute value disagreement according to \eqref{eq:disagreement}
  \State $d_{1:l} \leftarrow \textrm{disagreement}(g_{1:l}; V_{1:m}$)
  \State Normalize to a probability distribution
  \State $\mathcal{C}_k(g_{1:l}) \equiv d_{1:l} \leftarrow d_{1:l}/\textrm{Norm}(d_{1:l})$
  \For {$i$=1,2,..$N_\text{episodes}$} \Comment {Student epoch}
  \State Sample $g_i \sim \mathcal{C}_k$
  \State Collect a trajectory under $\tau_{k,i} = \phi^k_\theta(.,g_i)$
  \State Store transition data into replay buffer
  \State $R \leftarrow \tau_{k,i}$
  \EndFor
  \ForAll{$\phi \in \{\phi_1, ..., \phi_m\}$}
    \State Perform Bellman-update according to \eqref{eq:bellman} on samples drawn from $R$
  \EndFor
  \State Update policy $\pi_\theta$ using any RL algorithm
  \EndFor
  \State {\bf Return: }{$\theta$}
\end{algorithmic}
\end{algorithm}

